ScaLA: Accelerating Adaptation of Pre-Trained Transformer-Based Language Models via Efficient Large-Batch Adversarial Noise

In recent years, large pre-trained Transformer-based language models have led to dramatic improvements in many natural language understanding tasks. To train these models with increasing sizes, many neural network practitioners attempt to increase the batch sizes in order to leverage multiple GPUs to improve training speed. However, increasing the batch size often makes the optimization more difficult, leading to slow convergence or poor generalization that can require orders of magnitude more training time to achieve the same model quality. In this paper, we explore the steepness of the loss landscape of large-batch optimization for adapting pre-trained Transformer-based language models to domain-specific tasks and find that it tends to be highly complex and irregular, posing challenges to generalization on downstream tasks. To tackle this challenge, we propose ScaLA, a novel and efficient method to accelerate the adaptation speed of pre-trained transformer networks. Different from prior methods, we take a sequential game-theoretic approach by adding lightweight adversarial noise into large-batch optimization, which significantly improves adaptation speed while preserving model generalization. Experiment results show that ScaLA attains 2.7--9.8$\times$ adaptation speedups over the baseline for GLUE on BERT-base and RoBERTa-large, while achieving comparable and sometimes higher accuracy than the state-of-the-art large-batch optimization methods. Finally, we also address the theoretical aspect of large-batch optimization with adversarial noise and provide a theoretical convergence rate analysis for ScaLA using techniques for analyzing non-convex saddle-point problems.

==> Makefile <==
PAPER=main

all: pdf
pdf: $(PAPER).pdf

SECTIONS = \
	evaluation.tex

TEXT = $(SECTIONS) 

TEX = main.tex \
        $(TEXT)

$(PAPER).bbl: references.bib
	export TEXINPUTS=.:./latex-styles:; \
	pdflatex $(PAPER); bibtex $(PAPER); pdflatex $(PAPER); pdflatex $(PAPER)

$(PAPER).pdf: $(TEX) $(FIGS) $(PAPER).bbl
	export TEXINPUTS=.:./latex-styles:; \
	pdflatex $(PAPER); bibtex $(PAPER); pdflatex $(PAPER); pdflatex $(PAPER)

clean:
	/bin/rm -f $(PAPER).aux $(PAPER).bbl $(PAPER).blg $(PAPER).dvi \
	$(PAPER).log $(PAPER).ps $(PAPER).pdf $(PAPER).out




==> _s7_ack.tex <==
\section*{Contributions}
\label{sec:contribution}

\noindent\textbf{SR} designed the NLG training experiments and architected the inference system.

\noindent\textbf{CL} led the NLG training experiments (Section~\ref{sec:standard_moe}) and contributed to Section~\ref{sec:moe_parameter_efficiency}.

\noindent\textbf{ZY} led the design and experiments of PR-MoE, and its system support (\sref{sec:pr_moe}).
% , contributed to the training framework, contributed to the discussion about MoS and its related experiments (\sref{sec:mos}).

\noindent\textbf{MZ} led the design and experiments of MoS (Section~\ref{sec:mos}) and memory-efficient checkpointing. 

\noindent\textbf{RYA} and \textbf{AAA} led the development and experiments of the inference system (Section~\ref{sec:optimizing_moe_inference_latency}).
%the core optimization of the MoE inference pipeline, including kernel development and several customized communication such as parallelism-coordinated communication and expert-slicing in order to run MoE-inference on large-scale GPU-clusters. Helped with running inference experiments on different number of GPUs and with different MoE model structures (Section~\ref{sec:optimizing_moe_inference_latency}).

%\noindent\textbf{AAA}

\noindent\textbf{JR} developed, debugged and integrated multiple software features into DeepSpeed.

\noindent\textbf{YH} designed, managed and led the overall research project.

\section*{Acknowledgment}
We thank Olatunji Ruwase from the Microsoft DeepSpeed Team for his contributions on developing, debugging, testing, and releasing the DeepSpeed-MoE software.
This work was done in collaboration with Brandon Norick, Zhun Liu, and Xia Song from the Microsoft Turing Team, Young Jin Kim, Alex Muzio, and Hany Hassan Awadalla from the Microsoft Z-Code Team, and both Saeed Maleki and Madan Musuvathi from the Microsoft SCCL team. 


==> convergence.tex <==
%\vspace{-2mm}
%\section{Theoretical Convergence Analysis}
%\label{sec:eval}
%\vspace{-2mm}
%\textbf{Background, Notation and Assumptions: }
%Let $f: \mathbb{X} \times \mathbb{Y} \to \mathbb{R}$ where $\mathbb{X} \subset \mathbb{R}^{d_X}, \mathbb{Y} \subset \mathbb{R}^{d_Y}$ are compact.
%We consider the general problem of a two-player sequential game represented as nonconvex-nonconcave minimax optimization that is stochastic with respect to the outer (first) player playing $x \in \mathbb{X}$ while sampling $\xi$ from $Q$ and deterministic with respect to the inner (second) player playing $y \in \mathbb{Y}$, i.e.,
%$
%\begin{align}
%\min_{x} \max_{y} \mathbb{E}_{\xi \sim Q}[f(x, y, \xi)] := \min_{x} \mathbb{E}_{\xi \sim Q}[g(x, \xi)]
%\end{align}
%$. 
%where the result of the inner maximization is denoted by $g(x) := \max_y f(x, y, \xi)$.
%Since finding the Stackelberg equilibrium, i.e., the global solution to the saddle point problem, is NP-hard, we consider the optimality notion of a \textit{local minimax} point~\cite{jin2020local}. Since maximizing over $y$ may result in a non-smooth function even when $f$ is smooth, %, unlike non-convex optimization,
%the norm of the gradient is not particularly a suitable metric to track the convergence progress of an iterative minimax optimization procedure. Hence, we use the gradient of the \textit{Moreau envelope}~\cite{davis2019stochastic} as the appropriate potential function.
%Let $\mu \in \mathbb{R}_+^h$. The $\mu$-Moreau envelope for a function $g: \mathbb{X} \to \mathbb{R}$ is defined as $g_{\mu}(x) := \min_z g(z) + \sum_{i=1}^h \frac{1}{2 \mu^i} \| x^i-z^i \|^2$. % and $\xi$ refers to samples from $Q$.
%(mini-batches) generated 
%Let $\phi(x, z) := g(z) + \sum_{i=1}^h \frac{1}{2 \mu^i} \| x^i-z^i \|^2$. 
%an infimal convolution 
\begin{comment}
Let $\mu \in \mathbb{R}_+^h$. The $\mu$-Moreau envelope for a function $g: \mathbb{X} \to \mathbb{R}$ is defined as $g_{\mu}(x) := \min_z g(z) + \sum_{i=1}^h \frac{1}{2 \mu^i} \| x^i-z^i \|^2$.
\end{comment}
% \minjia{What's the importance of saying "infimal convolution" here? Can we remove it? \\
% Niranjan: Sure, addressed!}
%The gradient of the Moreau envelope is given by $\nabla_x [g_{\mu}(x)] =  \left[ \frac{1}{\mu^1} \left( x^1 - \arg \min_{z^1} \phi(x, z) \right), \ldots,  \frac{1}{\mu^h} \left( x^h - \arg \min_{z^h} \phi(x, z) \right) \right]$.
%Another reason for the choice of this potential function is due to the special property~\cite{rockafellar2015convex} of the Moreau envelope that if its gradient $\nabla_x [g_{\mu}(x)]$ almost vanishes at $x$, such $x$ is close to a stationary point of the original function $g$ (details in Appendix~\ref{sec:proof}).
%\textbf{TODO}Our convergence guarantee moreau cdorresponds to original space result

% \minjia{We are exceeding the page limit a lot, and I'm considering moving some contents to the appendix. It seems the Moreau envelope is used only in the proof. I wonder if we could move some of the content above to the appendix but perhaps mention them briefly in the main paper. \\
% Niranjan: Sure, addressed!}

%For any $m \in \mathbb{R}$, the function $\nu: \mathbb{R} \rightarrow [\mathcal{L}, \mathcal{U}]$ clips its values, i.e., $\mathcal{L} \leq \nu^i(m) \leq \mathcal{U}, \forall i \in [h]$.
%We denote the minimum value of the outer minimization as $g(x^*) := \min_x g(x)$.
%we show that 
% Let $t_s =0$. Under these assumptions, \name achieves an error tolerance of $\epsilon$ in $\widetilde{O}(\kappa_\alpha^2 \epsilon^{-2})$ iterations (proofs in Appendix~\ref{sec:proof}).% For simplicity, we present the zero momentum case (Theorem~\ref{lem:lars}).

%For simplicity, we analyze the zero momentum case (Lemma~\ref{lem:lars}).
%Under the above assumptions, s
\begin{theorem}[Complexity of Algorithm~\ref{algo:algorithm}; Informal -- Details in Appendix~\ref{sec:proof}]
\label{thm:oracle}
Consider the problem in Equation~\ref{eqn:formulation}. Let $t_s =0$. Setting the outer learning rate as $\eta = O \left( 1 / \sqrt{T} \right)$ and scaling batch size as $b = O(T)$, for Algorithm~\ref{algo:algorithm}, we have
%\begin{align}
$
    \mathbb{E} \left[ \| \nabla g_{1/2 \alpha}(\overline{x}) \|^2 \right] \leq O \left( \epsilon  + \kappa_\alpha / \sqrt{T} \right)
$
%\end{align}
% \minjia{There is "misplaced alignment tab character \&" error in the above equation. Please fix it. \\
% Niranjan: Sure, addressed!}
where $\overline{x}$ is the estimator obtained from running $T$ steps of Algorithm~\ref{algo:algorithm} and picking $x_t$ uniformly at random for $t \in [T]$. Here, $\epsilon$ is the error due to the approximate inner maximization oracle, $\alpha$ characterizes the smoothness of $f(x,.)$, $g_{1/2\alpha}$ is the Moreau-envelope of $g$ and $\kappa_\alpha = \max_i \alpha_i / \min_i \alpha_i$.
\end{theorem}
% which also matches previously known bounds~\cite{lin2020gradient}.
%\begin{theorem}[Oracle-free complexity, informal]
%\label{thm:oracle_free}
%\end{theorem}


